Semi-classical predictions of cosmological wave-packets from ridge-lines

We introduce a concept of ridge-lines to investigate the semi-classical prediction from wave-packets with arbitrary width in conventional quantum mechanics and the Wheeler--DeWitt quantum cosmology. Two primary approaches are applied to the exact calculation of the ridge-lines, namely the contour and the stream approach. Moreover, aspects of these are discussed and compared to other scenarios and approaches, i.e. the narrow WKB wave-packets and the first-derivative test. As the main result, we show that the semi-classical predictions in toy models have more abundant solutions than in the classical theory, and most interestingly they may deviate from classical solutions due to the quantum corrections.

==> tikz/moments.tex <==
\begin{tikzpicture}
\begin{axis}[
	ymode=log,
	xlabel=$n$,
	ylabel=$\abr{\nu^n}$,
	xmin=-.5,
	xmax=16.5,
	legend pos=north west,
]

\addplot+[
	only marks
	] table {./data/moments1.dat};
\addplot+[
	only marks
	] table {./data/moments2.dat};

\legend{$\mscrA_{\text{lin}}$, $\mscrA_{\text{hfg}}$},

\end{axis}
\end{tikzpicture}

